Green functions and twist correlators for $N$ branes at angles

We compute the Green functions and correlator functions for N twist fields for branes at angles on T^2 and we show that there are N-2 different configurations labeled by an integer M which is roughly associated with the number of obtuse angles of the configuration. In order to perform this computation we use a SL(2,R) invariant formulation and geometric constraints instead of Pochammer contours. In particular the M=1 or M=N-1 amplitude can be expressed without using transcendental functions. We determine the amplitudes normalization from N -> N-1 reduction without using the factorization into the untwisted sector. Both the amplitudes normalization and the OPE of two twist fields are unique (up to one constant) when the \epsilon <-> 1-\epsilon symmetry is imposed. For consistency we find also an infinite number of relations among Lauricella hypergeometric functions.

==> diff_NPBv1_V1 <==
128c128
< with the number of reflex angles of the configuration.
---
> with the number of obtuse angles of the configuration.
178c178
< (\cite{Bianchi:1991rd}, \cite{Gava:1997jt}, \cite{David:2000um},
---
> (\cite{Gava:1997jt}, \cite{David:2000um},
185c185
< and that the number of sectors is equal to the number of reflex angles
---
> and that the number of sectors is equal to the number of obtuse angles
193c193
< \input{6gons.tex}
---
> \input{6gons.pdf_tex}
210c210
< approach in (\cite{Anastasopoulos:2011gn}, \cite{Anastasopoulos:2011hj}). 
---
> approach in \cite{Anastasopoulos:2011gn}. 
290c290
< \input{Map_stripe_polygon.tex}
---
> \input{Map_stripe_polygon.pdf_tex}
357c357
< \input{angles_v1_ridotto.tex}
---
> \input{angles_v1_ridotto.pdf_tex}
374c374
<      \input{N_4Sigma_w_angles.tex}
---
>      \input{N_4Sigma_w_angles.pdf_tex}
376c376
<      \caption{A polygon $\Sigma$ with an reflex angle and branes counted
---
>      \caption{A polygon $\Sigma$ with an obtuse angle and branes counted
384c384
<      \input{N_4Sigma_w_angles_clockwise.tex}
---
>      \input{N_4Sigma_w_angles_clockwise.pdf_tex}
386c386
<      \caption{A polygon $\Sigma$ with an reflex angle and branes
---
>      \caption{A polygon $\Sigma$ with an obtuse angle and branes
784c784
< \input{omega_cuts.tex}
---
> \input{omega_cuts.pdf_tex}
831c831
< this integer $M$ is equal to the number of reflex angles plus 2 since
---
> this integer $M$ is equal to the number of obtuse angles plus 2 since
833,834c833,834
< while every reflex one is $2\pi-\pi\epsilon$
< as shown in fig. (\ref {fig:Acute-Reflex-Contribution}).
---
> while every obtuse one is $2\pi-\pi\epsilon$
> as shown in fig. (\ref {fig:Acute-Obtuse-Contribution}).
840c840
< \input{Acute-Obtuse-contribution.tex}
---
> \input{Acute-Obtuse-contribution.pdf_tex}
846,847c846,847
< $\pi-\pi\epsilon$ while an reflex one  to $2\pi-\pi\epsilon$. }
< \label{fig:Acute-Reflex-Contribution}
---
> $\pi-\pi\epsilon$ while an obtuse one  to $2\pi-\pi\epsilon$. }
> \label{fig:Acute-Obtuse-Contribution}
863c863
< \input{difference_of_f_and_angle.tex}
---
> \input{difference_of_f_and_angle.pdf_tex}
884c884
< of reflex angles must be less or equal than $N-3$ we deduce that $
---
> of obtuse angles must be less or equal than $N-3$ we deduce that $
898c898
< \input{N4M2Sigma_w_various_D4_shifts_all_pics_1line.tex}
---
> \input{N4M2Sigma_w_various_D4_shifts_all_pics_1line.pdf_tex}
912c912
< \input{N4M3Sigma_w_various_D4_shifts_all_pics_1line.tex}
---
> \input{N4M3Sigma_w_various_D4_shifts_all_pics_1line.pdf_tex}
1343,1387c1343,1345
< the case $M=N-2$ and there is not any difference among the different
< $M$ values therefore the results obtained there are valid.
< Let us anyhow quickly review them.
< Given a minimal $N$-polygon in $T^2$ with vertexes $\{f_i\}$,
< i.e. with all vertexes in the fundamental cell,  
< we can consider non minimal polygons which wrap the $T^2$.
< These can be easierly described
< as polygons which have vertexes $\{ \tilde f_i \}$ 
< in the covering $\R^2$ where $T^2 \equiv R^2 / \Lambda$ with
<  the lattice defined as $\Lambda=\{ n_1 e_1+ n_2 e_2 | n_1,n_2\in \Z\}$.
< These configurations give an additive contribution to the classical
< path integral as
< \begin{align}
< \langle 
< \sigma_{\epsilon_1,f_1}(x_1) \dots \sigma_{\epsilon_N,f_N}(x_N)
< \rangle_{T^2}
< =
< \cN(x_i,\epsilon_i)
< \sum _{\{\tilde  f_i\}}
<  e^{-S_{E,cl}(x_i,\epsilon_i, \tilde f_i)}
< \label{general_corr_from_quantum_and_classical_on_T2}
< \end{align}
< % $e^{-S_{cl}(f_i)}\rightarrow \sum _{\{\tilde  f_i\}}e^{-S_{cl}(\tilde f_i)}$.
< 
< In order to determine the possible vertexes  $\{ \tilde f_i \}$
< without redundancy it is necessary to keep a vertex fixed and then
< expand the polygon. For definiteness we keep fixed the vertex $\tilde f_1=f_1$ 
< which lies at the intersection between $D_N$ and $D_1$.
< We then move the next vertex $f_2$ along the $D_1$ brane. 
< Explicitly we write $\tilde f_2= \tilde f_1+ (f_2-f_1) + n_1 t_1= 
< f_2+ n_1 t_1$ with $n_1\in \Z$ and
< $t_1$  the shortest tangent vector to $D_1$ which is in $\Lambda$.
< We can now continue for all the other vertexes for which we have
< $\tilde f_i = \tilde f_{i-1} +( f_{i}-f_{i-1})+ n_{i-1} t_{i-1}
< =f_i + \sum_{k=1}^{i-1} n_k t_k$.
< For consistency we need requiring $\tilde f_{N+1} \equiv \tilde f_1 =
< f_1$,
< therefore the possible wrapped polygons are obtained from the solution
< of the Diophantine equation
< \begin{align}
< \sum_{i=1}^N n_i t_i =0
< \end{align}
< which cannot be solved in general terms but only on a case by case
< basis as discussed in \cite{Abel:2003yx}.
<    
---
> the case $M=N-2$ and
> there is not any difference among the different $M$ values therefore
> the results obtained there are valid. 
3155,3158c3113
< W_{S,\bS}$, explicitly we find\footnote{See appendix
<   \ref{app:details_reductions}
< for an example of the computations involved in the special case $N=4$ $M=2$.
< }
---
> W_{S,\bS}$, explicitly we find
3562,3564d3516
< \noindent {\large {\bf Acknowledgments}}
< We thank M. Bianchi for pointing out a mistake in a figure.
< 
3585c3537
< First we interpret the previous integral in $y$ as a line integral in
---
> First we interpret the previous integral in $y$ as a path integral in
3602c3554
< \input{KLT_phases.tex}
---
> \input{KLT_phases.pdf_tex}
3659c3611
< \input{KLT_phase_eta_plane.tex}
---
> \input{KLT_phase_eta_plane.pdf_tex}
3687c3639
< \input{KLT_path_single_point.tex}
---
> \input{KLT_path_single_point.pdf_tex}
3821,3946d3772
< \section{Some details on the $N=4$ reduction}
< \label{app:details_reductions}
< As an example of the way we performed the $N\rightarrow N-1$ we give
< now some details on the $N=4$ $M=2$ case, in particular 
< we consider $\omega_3 \rightarrow 0$ when $\theta_3+\theta_4>1$.
< Under this conditions we want to compute the behavior of
< \begin{align}
< \det W=
< \left|
< \begin{array}{c c}
< W^3_1 & W^{\bar 3}_1 \\
< W^3_2 & W^{\bar 3}_2 
< \end{array}
< \right|
< \end{align}
< where we have chosen $S=\bar S=\{3\}$.
< The different entries of the determinant have the following limits
< \begin{align}
< W^3_1
< &=
< \int^{1}_{\omega_3} d \omega 
< ~(\omega-1)^{\theta_2-1}
< ~(\omega-\omega_3)^{\theta_3-1}
< ~\omega^{\theta_4-1}
< \sim
< \int^{1}_{0} d \omega 
< ~(\omega-1)^{\theta_2-1}
< ~\omega^{(\theta_3+\theta_4-1)-1}
< \\\noindent
< &= 
< e^{i \pi (\theta_2 -1)}
< B(\theta_2, \theta_3+\theta_4-1),
< \end{align}
< 
< \begin{align}
< W^3_2
< &=
< \int^{\omega_3}_0 d \omega 
< ~(\omega-1)^{\theta_2-1}
< ~(\omega-\omega_3)^{\theta_3-1}
< ~\omega^{\theta_4-1}
< \nonumber\\
< &=
< \omega_3^{\theta_3+\theta_4-1}
< \int^{1}_{0} d t
< ~(\omega_3 t -1)^{\theta_2-1}
< ~(t-1)^{\theta_3-1}
< ~t^{\theta_4-1}
< \nonumber\\
< &\sim 
< \omega_3^{\theta_3+\theta_4-1}
< ~e^{i \pi(\theta_2+\theta_3)}
< ~B(\theta_3, \theta_4),
< \end{align}
< and
< \begin{align}
< W^{\bar 3}_1
< &=
< \int^1_{\omega_3} d \omega 
< ~(\omega-1)^{-\theta_2}
< ~(\omega-\omega_3)^{-\theta_3}
< ~\omega^{-\theta_4}
< \nonumber\\
< &=
< \omega_3^{1-\theta_3-\theta_4}
< \int^{1/\omega_3}_{1} d t
< ~(\omega_3 t -1)^{-\theta_2}
< ~(t-1)^{-\theta_3}
< ~t^{-\theta_4}
< \nonumber\\
< &
< \sim 
< ~e^{-i \pi\theta_2}
< \omega_3^{1-\theta_3-\theta_4}
< \int^{+\infty}_{1} d t
< ~(t-1)^{-\theta_3}
< ~t^{-\theta_4}
< =
< ~e^{-i \pi\theta_2}
< \omega_3^{1-\theta_3-\theta_4}
< ~B(\theta_3+\theta_4-1, 1-\theta_3)
< \end{align}
< finally the limit of the last entry can be obtained using 
< again the substitution $\omega=\omega_3 t$ to be
< \begin{align}
< W^{\bar 3}_2
< &=
< \int^{\omega_3}_0 d \omega 
< ~(\omega-1)^{-\theta_2}
< ~(\omega-\omega_3)^{-\theta_3}
< ~\omega^{-\theta_4}
< \sim
< ~e^{-i \pi(\theta_2+\theta_3)}
< \omega_3^{1-\theta_3-\theta_4}
< ~B(1-\theta_3, 1-\theta_4)
< \end{align}
< Inserting all the previous asymptotic behaviors into the determinant
< we get its $\omega_3 \rightarrow 0$, $\theta_3+\theta_4>1$ limit to be
< \begin{align}
< \det W
< &=
< \left|
< \begin{array}{c c}
< B(\theta_2, \theta_3+\theta_4-1) 
< & 
< \omega_3^{1-\theta_3-\theta_4}
< ~B(\theta_3+\theta_4-1, 1-\theta_3)
< \\
< \omega_3^{\theta_3+\theta_4-1}
< ~e^{i \pi(\theta_3-1)}
< ~B(\theta_3, \theta_4)
< & 
< \omega_3^{1-\theta_3-\theta_4}
< ~B(1-\theta_3, 1-\theta_4)
< \end{array}
< \right|
< \nonumber\\
< &\sim
< \omega_3^{(1-\theta_3)+(1-\theta_4)-1}
< ~B(1-\theta_3, 1-\theta_4)
< ~B(\theta_2, 1-(1-\theta_3)-(1-\theta_4)) 
< \end{align}
< where it is worth noticing that we can drop the relative phases since
< only one product is the leading one. This happens luckily also for all
< the other computations which are needed to compute all the $N
< \rightarrow N-1$ reduction.
4033,4047d3858
< %\cite{Anastasopoulos:2011hj}
< \bibitem{Anastasopoulos:2011hj}
<   P.~Anastasopoulos, M.~Bianchi and R.~Richter,
<   ``Light stringy states,''
<   JHEP {\bf 1203} (2012) 068
<   [arXiv:1110.5424 [hep-th]].
<   %%CITATION = ARXIV:1110.5424;%%
< 
< %\cite{Bianchi:1991rd}
< \bibitem{Bianchi:1991rd}
<   M.~Bianchi, G.~Pradisi and A.~Sagnotti,
<   ``Planar duality in the discrete series,''
<   Phys.\ Lett.\ B {\bf 273} (1991) 389.
<   %%CITATION = PHLTA,B273,389;%%
< 
4075c3886
<   [arXiv:1101.5898 [hep-th]].\\
---
>   [arXiv:1101.5898 [hep-th]].
4077,4084d3887
< %\cite{Pesando:2008xt}
< %\bibitem{Pesando:2008xt}
<   I.~Pesando,
<   %``A Comment on discrete Kalb-Ramond field on orientifold and rank reduction,''
<   Phys.\ Lett.\ B {\bf 668} (2008) 324
<   [arXiv:0804.3931 [hep-th]].
<   %%CITATION = ARXIV:0804.3931;%%
< 

